High-Resolution, Respiratory-Resolved Coronary MRA Using a Phyllotaxis-Reordered Variable-Density 3D Cones Trajectory

Purpose: To develop a respiratory-resolved motion-compensation method for free-breathing, high-resolution coronary magnetic resonance angiography using a 3D cones trajectory. Methods: To achieve respiratory-resolved 0.98 mm resolution images in a clinically relevant scan time, we undersample the imaging data with a variable-density 3D cones trajectory. For retrospective motion compensation, translational estimates from 3D image-based navigators (3D iNAVs) are used to bin the imaging data into four phases from end-expiration to end-inspiration. To ensure pseudo-random undersampling within each respiratory phase, we devise a phyllotaxis readout ordering scheme mindful of eddy current artifacts in steady state free precession imaging. Following binning, residual 3D translational motion within each phase is computed using the 3D iNAVs and corrected for in the imaging data. The noise-like aliasing characteristic of the combined phyllotaxis and cones sampling pattern is leveraged in a compressed sensing reconstruction with spatial and temporal regularization to reduce aliasing in each of the respiratory phases. Results: In a volunteer and 5 patients, respiratory motion compensation using the proposed method yields improved image quality compared to non-respiratory-resolved approaches with no motion correction and with 3D translational correction. Qualitative assessment by two cardiologists indicates the superior sharpness of coronary segments reconstructed with the proposed method (P < 0.01). Conclusion: The proposed method better mitigates motion artifacts in free-breathing, high-resolution coronary angiography exams compared to translational correction.

==> figs_copy.tex <==
\newpage

FIG 1. Traditional algorithms for non-Cartesian regularized SENSE implicitly estimate a convolution with the sampling point spread function every iteration using nonuniform Fourier transforms (NUFFTs) (top row). The Toeplitz-based method computes a circular convolution over twice the image size using a transfer function represented in Cartesian coordinates (Eq. \ref{eq:Mdef_a}), which produces an identical result within the original image size provided that the object is bounded. Cropping after circular convolution eliminates the erroneous result outside the original image size (Eq. \ref{eq:Mdef_a}).

FIG 2. The reconstruction times for the gradient computation (i.e., $S_N^HWS_N$ for NUFFT and $Z^HF^{-1}MFZ$ for Toeplitz) for both CPU and GPU implementations for various undersampling rates and image matrix size factors compared to the nominal matrix size of $128 \times 128 \times 64$. NUFFT oversampling was 1.5 and the kernel width was 4.

FIG 3. Rates of speed increase for Toeplitz compared to NUFFT for the gradient computation (i.e., $S_N^HWS_N$ for NUFFT and $Z^HF^{-1}MFZ$ for Toeplitz) for both CPU and GPU implementations. The left panels show trends as the kernel width and oversampling ratio are varied, while the undersampling rate is fixed at 4 and the FOV size factor relative to the nominal FOV of $128 \times 128 \times 64$ is fixed at 1.5. The right panel shows trends as the undersampling rate and size factor are varied, while the NUFFT oversampling and kernel width are fixed to 1.5 and 6, respectively. Timings for 3D cones and radial trajectories were averaged with each other before computing the speed increases (individual trends were similar).

FIG 4. (a) In some non-Cartesian acquisitions, signal may lie outside the FOV the trajectory was designed for, which can be assessed from calibration data using an ESPIRiT eigenvalue threshold. (b) Compressed sensing reconstructions that ignored the signal outside the nominal matrix size exhibited errors that were eliminated when the optimal size was used.

FIG 5. Normalized root-mean-square-error (RMSE) and number of iterations required to converge as $\kappa$ is varied from 0 to 1. Shown below are differences from ground truth for $\kappa=\{0, 0.3, 0.6, 1\}$ in a sample slice. There is little change in error, but large changes in convergence speed, for $\kappa$ near 0. The difference images are scaled by 10 for 3D cones and 20 for 3D radial, relative to the ground truth image shown on the bottom left (similar results in other slices). 
    











